A Simple yet Effective Self-Debiasing Framework for Transformer Models

Current Transformer-based natural language understanding (NLU) models heavily rely on dataset biases, while failing to handle real-world out-of-distribution (OOD) instances. Many methods have been proposed to deal with this issue, but they ignore the fact that the features learned in different layers of Transformer-based NLU models are different. In this paper, we first conduct preliminary studies to obtain two conclusions: 1) both low- and high-layer sentence representations encode common biased features during training; 2) the low-layer sentence representations encode fewer unbiased features than the highlayer ones. Based on these conclusions, we propose a simple yet effective self-debiasing framework for Transformer-based NLU models. Concretely, we first stack a classifier on a selected low layer. Then, we introduce a residual connection that feeds the low-layer sentence representation to the top-layer classifier. In this way, the top-layer sentence representation will be trained to ignore the common biased features encoded by the low-layer sentence representation and focus on task-relevant unbiased features. During inference, we remove the residual connection and directly use the top-layer sentence representation to make predictions. Extensive experiments and indepth analyses on NLU tasks show that our framework performs better than several competitive baselines, achieving a new SOTA on all OOD test sets.

==> content/experiments-v1.tex <==
\section{Experiments}
\label{sec:experiments}

\subsection{Experimental Setup}
\label{ssec:experiment-setup}

\paragraph{Tasks and Datasets}
To verify the effectiveness of our framework, we conduct several groups of experiments on three common NLU tasks: natural language inference, paraphrase identification and fact verification. 
For each task, we use its existing challenge test sets for evaluation, where their bias information is not used for model training. 
In the following, we give a brief description for each task, including the biased datasets for training and the corresponding challenge test sets for debiasing evaluation. 

\begin{itemize}
\item \textbf{Natural Language Inference (NLI)} is to predict the entailment relationship between the pair of premise and hypothesis. We build NLI models using the MNLI dataset \cite{ DBLP:conf/naacl/WilliamsNB18}, and evaluate them on the corresponding challenging test set HANS \cite{hans2019}. HANS is designed to test whether NLI models make predictions on three fallible syntactic heuristics: the lexical overlap heuristic, the subsequence heuristic, and the constituent heuristic.

\item \textbf{Paraphrase Identification (ParaIden)} is to predict whether the given question pair is \textit{duplicate} or \textit{non-duplicate} in semantics. We use the QQP dataset\footnote{https://www.kaggle.
com/c/quora-question-pairs} to train models, and evaluate model performance on the challenge set PAWS \cite{zhang-etal-2019-paws}, which investigates whether the model exploits word overlapping features to make predictions.

\item \textbf{Fact Verification (FactVer)} aims to identify whether a textual claim is supported or refuted by the given evidence text. We adopt the FEVER dataset \cite{thorne2018fact} to train models, and assess the model abilities on FeverSymmetric (\textit{Symm.}) \cite{feversymm2019}, which is created to reduce claim-only biases.
\end{itemize}

The basic statistics of all datasets used in our experiments are shown in Table \ref{tab:data_statistics}.

\input{table/datasets_statistics}

\input{table/main_results}

\paragraph{Baselines}
\textcolor{red}{Most of previous debiasing frameworks involve two stages, namely biased sample identification and debiasing models. We select two popular methods for biased sample identification and three debiasing methods. And we report results of their combinations in Table \ref{tab:main_results}. }
%We select several competitive models as our baselines:
\begin{itemize}
\item \textbf{Known-Bias (Manual bias identification)} \cite{gururangan-etal-2018-annotation, utama-etal-2020-mind, du-etal-2021-towards} quantifies the bias degree of each training sample via data statistics or researchers' insights. Then the instances with high bias degree are taken as biased instances and often used to train a bias-only model. 

   

\item \textbf{Self-debias (Bias automatic identification)} \cite{utama-etal-2020-towards} trains a low capacity model based on a small part of the training data to automatically identify biased instances, where this model is also used as the bias-only model. 

\item \textbf{ER (Re-weighting)} \cite{ clark-etal-2019-dont} aims to reduce contributions of biased instances on the overall training loss by assigning a scalar weight on their losses. For example, the scalar weight in \citet{clark-etal-2019-dont} is computed as $1-p^i_b$, where $p^i_b$ is output by the bias-only model for the $i$-th example. 

\item \textbf{PoE (Product-of-expert)} \cite{clark-etal-2019-dont} trains the main model in an ensemble with the bias-only model which is trained in advance and uses biased features to make predictions. With this manner, the main model is encouraged to focus on unbiased features and much robust.

\item \textbf{CR (Confidence Regularization)} \cite{utama-etal-2020-mind} trains a bias-only model and a teacher model, where the output probability distribution of the latter is scaled by that of the former. Then the re-scaled output distribution is used to distill the main model.


\item \textbf{End2End} \citet{ghaddar-etal-2021-end} propose an end-to-end framework for bias identification and debiasing. They train a shallow model on the representations of a low layer and a main model on the top layer. The two models are trained simultaneously and they interact by interchangeably re-weighting the importance of each others' instances.
\end{itemize}
\iffalse
\begin{itemize}
    \item 
    \textbf{BERT}. We use the training data to fine-tune BERT-based model; 
    \item 
    \textbf{Example Reweighting (ER)} \cite{schuster-etal-2019-towards}. In this variant, biased instances are assigned with small weights to reduce their impacts on the training loss;
    \item
    \textbf{Product-of-expert (PoE)} \cite{clark-etal-2019-dont}. It first train a bias-only model to identify biased instances, and then train the robust model as part of an ensemble with the naive one in order to encourage it to focus on unbiased features.
    \item 
    \textbf{Confidence Regularization (CR)} \cite{utama-etal-2020-mind}. It first builds a bias-only model and a teacher model, and then use the predicted probabilities from bias-only model to regularize those from the teacher model. The robust model is trained by these regularized probabilities;
    \item
    \textbf{Unknown Biases (UB)} \cite{utama-etal-2020-towards}.    It first uses some portions of training data to train a bias-only model, and then utilize the bias-only model to conduct debiasing in a PoE manner.
    \item
    \textbf{Self Debiasing (SD)} \cite{ghaddar-etal-2021-end}.
    It adds a classifier to the lower layer of model.
    instances with high probabilities predicted by lower layer are treated as biased ones, of which impacts on training loss are reduced.
\end{itemize}
\fi


\paragraph{Evaluation Metrics}
\textcolor{red}{For each task, following \citet{utama-etal-2020-towards}, we evaluate model performance on the original dev set and the corresponding challenge test set. Similarly, we use accuracy (\textit{Acc.}) as the main metric for tasks of NLI and fact verification, and use F1-score (\textit{F1}) for the task of paraphrase identification. 
In addition, we evaluate interpretability results on the QQP dataset with metrics defined in \citet{wang2022fine}. Please see Section \ref{ssec:result-analysis} for details.}
 
\paragraph{Our Implementations}
\textcolor{red}{We implement our proposed framework on the BERT base model, which has shown impressive in-distribution performance on the three tasks. During fine-tuning models on each dataset, we follow the standard setup for input construction and use the representation of token [CLS] for classification. For each task, we use a batch size of 32 and fine-tune for 5 epochs with the learning rate 5e-5. Besides, we take Adam \cite{DBLP:journals/corr/KingmaB14} as the optimizer. 
To learn the biased representations, we set the low layer $b$ as 4.}

Meanwhile, we provide a variant of our framework (i.e., debiasing with residual connection, DeRC). Following the previous two-stage frameworks, we use the output probabilities of the low layer to identify biased instances, and apply PoE based method for debiasing models, denoted as \textbf{DePoE}. 

\iffalse
\begin{itemize}
    \item \textbf{Debiasing with Residual Connection (DeRC)}. It is the basic model described in Section \ref{sec:debiasing-framework}.
    \item
    \textbf{Debiasing with Product-of-Experts (DePoE)}.
    In this variant, the predicted probabilities instead of representations of lower layer are used to debias the representation learning of top layer, following a similar way as PoE.
    \item
    \textbf{Debiasing with No Additional Parameters (DeNAP)}.
    It reuses the classifier of top-layer to transform the representations of lower layer into probabilities. Note that we do not use $\mathcal{L}_b$ to update the classifier parameters to avoid influencing the training of top-layer. Besides, it contains exactly the same number of parameters as BERT.
\end{itemize}
\fi
\paragraph{Effect of the Chosen Layer \textbf{$l_b$}} As described in Section \ref{}, the chosen layer $l_b$ is an important hyper-parameter in our framework. To investigate the effect of $l_b$, we vary $l_b$ from 1 to 6 and report the performance of corresponding \textit{DeRC} on the challenge sets of three tasks.
As shown in Figure \ref{}, when $l_b$ equals as $\{4, 5, 6\}$, \textit{DeRC} consistently surpass the previous best results in all three tasks, indicating that we are not required to carefully search the optimal $l_b$ for each task. Based on this, we set $l_b=3$ in all subsequent experiments.



\subsection{Main Results}
\label{ssec:main-results}
We show the experimental results in Table \ref{tab:main_results}, including results on the original dev sets and the challenge test sets. 
From the comparison between our proposed framework \textit{DeRC} and other debiasing frameworks, we can observe that \textit{DeRC} achieves the best performance on all challenge sets of three tasks, setting a new SOTA. In particular, \textcolor{red}{on the PAWS dataset, \textit{DeRC} improves F1 score by 11.3, while the previous best work (PoE+Known-Bias) only brought a gain of 1.6. }
\textcolor{red}{Besides, by comparing results on the original dev sets, \textit{DeRC} brings the smallest performance drop on the QQP dataset, and achieves the largest accuracy improvement on FEVER. That is, our proposed framework is not only very effective in improving model performance in OD setting, but also harmless in ID setting. }
This strongly verifies the superiority of our proposed framework.

Furthermore, when considering our three variants, we find that \textit{DeRC} surpasses \textit{DePoE} on all three tasks. Note that \textit{DeRC} and \textit{DePoE} use the biased representations and biased probabilities for debiasing, repsectively, we confirm that leveraging the biased representation is a better solution. 


==> content/introduction-v1.tex <==
\section{Introduction}

While neural models have achieved amazing performance on many NLU (natural language understanding) benchmarks \cite{devlin-etal-2019-bert, wang-etal-2018-glue}, recent studies show that they tend to exploit dataset biases (i.e., spurious correlations between surface patterns and labels, as shown in Table \ref{tab:case_intro}) as shortcuts to make predictions, rather than reasonable reasoning on accurate understanding \cite{geirhos2020shortcut, gururangan-etal-2018-annotation, mccoy-etal-2019-right}. These biases result in the low generalizability and low robustness of neural models on out-of-distribution (OOD) samples \cite{zellers-etal-2018-swag}. For example, several challenge test sets such as HANS \cite{hans2019} and PAWS \cite{zhang-etal-2019-paws} are constructed to test model performance on the OOD setting, and lead to a performance drop of all the state-of-the-art (SOTA) models.

\input{table/bias-example.tex}

Consequently, some model-agnostic debiasing methods are proposed to mitigate the impact of biases, such as example re-weighting \cite{feversymm2019, schuster-etal-2019-towards, karimi-mahabadi-etal-2020-end}, confidence regularization \cite{utama-etal-2020-mind} and model ensemble \cite{clark-etal-2019-dont, he-etal-2019-unlearn, karimi-mahabadi-etal-2020-end}. They have improved the performance on challenge sets by down-weighting the importance of biased examples in the training loss. 
Meanwhile, many studies aim to unveil biased examples. Some works manually characterize the specific types of biases based on the assumption that the types of biases should be known a-priori \cite{gururangan-etal-2018-annotation, poliak-etal-2018-hypothesis, tsuchiya-2018-performance, schuster-etal-2019-towards}. Other works train an extra model to automatically identify potentially biased examples \cite{utama-etal-2020-towards, ghaddar-etal-2021-end, utama-etal-2020-mind}. 
However, few studies have utilized the internal structure of the model to identify and mitigate biases without knowing their types in advance or training additional models. Since neural models fine-tuned by transformer-based pre-trained language models have achieved SOTA performance on various NLP tasks \cite{devlin-etal-2019-bert, liu2019roberta}, understanding whether they have exploited shortcuts and to which degree they have learned is very important. Inspired by recent research on the effect of different layers in linguistic knowledge learning \cite{jawahar-etal-2019-bert, tenney-etal-2019-bert}, we propose two questions. Is the shortcut learning different in different layers of transformer architecture? Can we use the internal structure of transformer to alleviate the bias tendency. 

difficulty。 
To answer above questions, in this paper, we first conduct a preliminary experiment to explore the impact of biases in the dataset on the features of different layers of BERT（一般第一句话就需要把我们的主要工作给出来，后面可以详细说具体做法）. Specifically, we construct anti-bias set from the test set according to some heuristic rules（这里不用写这么细，直接给出结论，否则容易让别人陷入细节，觉得我们又跟历史工作一样了）. Then, using the features of each layer in BERT to predict sentence category. By analyzing the performance gap between differences layers on test set and anti-bias set, we find that compared with high layers, the low layers are more affected by anti-bias samples, which proves that the low layers of BERT tend to pay more attention to the shortcuts information than the high layers.

Then based on this observation, we further propose a debias model based on the residual connection （这里确定使用残差形式了吗，是否理得顺，是否要考虑一下）which allows the model predict label by using semantic understanding rather than shortcuts, so as to enhance the generalization ability of model.
Concretely, in the training phrase, we use the residual connection \cite{residual} to add the features of bottom layer, which learn the shortcuts of the dataset to the features of top layer, and use the new features to fit the golden truth label. By doing so, the model will be encouraged to pay more attention to the non-shortcuts information in the sample,
because the shortcuts have been provided by the bottom layer. In the inference phrase, we will remove the residual connection and directly use the top-level features for prediction. Compare with previous studies \cite{XXX}, our framework has the following advantages: 1) less computing resource consumption, the whole process of debias is completed in the same model; 2) fewer hyperparamters (only one hyperparameter), which means we have fewer restrictions; 3) our model is task-agnostic（这部分优点再考虑一下，跟下面的贡献有一些冲突了，可以看一下这段的细节，有没有必要放在正文中，而不是introduction中）.

Our contributions include:
\begin{itemize}[leftmargin=*]
\item Through experimental analysis, we verify that the features of each layer in BERT are affected by bias in different degrees. On the whole, with the deepening of the number of layers, the degree of influence is slowly decreasing;
\item Using the observation, we propose a debiasing method based on the residual connection, which adds the bottom-level features to the top-level features to urge the high-level of the model to pay attention to semantics. Compared with the previous work, this method is more simple and effective (only two lines of code need to be added), the task-agnostic, less hyper-parameter, and almost no additional parameters are introduced, which saves the consumption of computing resources;

\item We conduct experiments on three NLU tasks and six test sets. The results show that our dibiasing framework has achieved high performance not only on conventional test sets, but also on challenge test sets. Through in-depth analysis, we find that our debiasing framework improves the robustness and interpretability of the model. 
\end{itemize}

==> table/bias-example-v1.tex <==
\begin{table}[tb]
\small
\center
\scalebox{0.95} {
\begin{tabularx}{0.48\textwidth}{ l }
\toprule[1pt]
\makecell[c]{\textbf{Word overlap}} \\
\hline
\makecell[l]{\textit{text1.}: It was named after Malaysia 's third prime minister. \\ \textit{text2.}: It was named after third Malaysia 's former Prime Minister. \\ \textit{Predicted Label}: Similarity} \\ \textit{Golden Label}: Not Similarity \\
\hline
\makecell[l]{\textit{Prem.}: The \textcolor{red}{actor} was paid by the \textcolor{red}{judge}. \\ \textit{Hypo.}: The actor paid the judge. \\ \textit{Predicted Label}: Entailment} \\
\midrule[1pt]
\makecell[c]{\textbf{Contradiction-Word}} \\
\hline
\makecell[l]{\textit{Prem.}: Understanding is the key. \\ \textit{Hypo.}: Understanding is the most important. \\ \textit{Predicted Label}: Entailment} \\
\hline
\makecell[l]{\textit{Prem.}: Understanding is the key. \\ \textit{Hypo.}: Understanding is the most important and false is \textcolor{red}{not} true. \\ \textit{Predicted Label}: Contradiction} \\
\bottomrule[1pt]
\end{tabularx}
}
\caption{Several biased examples \cite{mccoy-etal-2019-right, zhou-bansal-2020-towards}. For each bias type, the first row shows the original instance, and the second row show the corresponding challenge one.}
\label{tab:case_intro}
\end{table} 


==> table/robustness.tex <==
\begin{table}[h]
\begin{tabular}{lcccc}
\hline
\multicolumn{1}{l|}{\multirow{2}{*}{}} & \multicolumn{2}{c|}{SA}                               & \multicolumn{2}{c}{STS}                               \\ \cline{2-5} 
\multicolumn{1}{l|}{}                  & \multicolumn{1}{c|}{base} & \multicolumn{1}{c|}{DeRC} & \multicolumn{1}{c|}{base} & DeRC                      \\ \hline
alternative dispensable words          & 92.15                     & 92.31                     & 91.60                     & 92.00                     \\ \hline
alternative important words            & 92.25                     & 93.22                     & 90.31                     & 91.53                     \\ \hline
syntax transformation                  & 89.00                     & 89.30                     & 94.87                     & 96.00                     \\ \hline
insert negative words                  & 83.41                     & 85.42                     & 92.00                     & 92.00                     \\ \hline
all types perturbations                & \multicolumn{1}{l}{89.19} & \multicolumn{1}{l}{90.06} & \multicolumn{1}{l}{92.19} & \multicolumn{1}{l}{92.88} \\ \hline
\end{tabular}
\caption{}
\label{tab:robustness}
\end{table}
